Low-Cost Outdoor Air Quality Monitoring and Sensor Calibration: A Survey and Critical Analysis

The significance of air pollution and the problems associated with it are fueling deployments of air quality monitoring stations worldwide. The most common approach for air quality monitoring is to rely on environmental monitoring stations, which unfortunately are very expensive both to acquire and to maintain. Hence environmental monitoring stations are typically sparsely deployed, resulting in limited spatial resolution for measurements. Recently, low-cost air quality sensors have emerged as an alternative that can improve the granularity of monitoring. The use of low-cost air quality sensors, however, presents several challenges: they suffer from cross-sensitivities between different ambient pollutants; they can be affected by external factors, such as traffic, weather changes, and human behavior; and their accuracy degrades over time. Periodic re-calibration can improve the accuracy of low-cost sensors, particularly with machine-learning-based calibration, which has shown great promise due to its capability to calibrate sensors in-field. In this article, we survey the rapidly growing research landscape of low-cost sensor technologies for air quality monitoring and their calibration using machine learning techniques. We also identify open research challenges and present directions for future research.

==> tables/appcomparison.tex <==
\begin{sidewaystable*}
    \centering
    \caption{Comparison of the different machine learning approaches for low-cost \acp{AQS} calibration, including performance measures and our evaluation criteria. For each pollutant, rows are ranked using our evaluation criteria-based final ranking in descending order.}
    \label{tab:appcomparison}
    \resizebox{\linewidth}{!}{\begin{tabular}{c | c | l | c c c c c c c c c c | c c c c | c c c c | c c c c c }
        \toprule
        Target & Method & Reference & \multicolumn{10}{ c|}{Features} & \multicolumn{4}{ c|}{Atmospheric features} & \multicolumn{4}{ c| }{Performance measures} & \multicolumn{5}{c}{Score} \\
         & & & CO & \ac{CO2} & NO & \ac{NOx} & \ac{NO2} & \ac{O3} & \ac{SO2} & VOCs & PM\textsubscript{2.5} & PM\textsubscript{10} & T & RH & AH & WS & RMSE & MAE & MAPE & $R^2$ & Reliability & Resolution & Accuracy & Technology & Final Score \\
        \midrule
        \multirow{8}{*}{CO} & MLR & \cite{Maag2016} & x &  &  &  & x & x &  &  &  &  & x & x &  &  & 0.048 ppm & NR & NR & NR & 
        5.00 & 5.00 & 3.90 & 2.33 & 4.03 \\
         & RF & \cite{Zimmerman2018} & x & x &  &  & x & x &  &  &  &  & x & x &  &  & NR & 7.9 ppb & NR & 0.99 & 
         2.17 & 4.00 & 5.00 & 2.50 & 2.43 \\
         & FFNN & \cite{Spinelle2017} & x & x &  &  & x &  &  &  &  &  & x &  & x &  & NR & 0.05--0.12 & NR & 0.367 & 
         2.43 & 5.00 & 3.38 & 1.00 & 2.24 \\
         & MLR & \cite{Zimmerman2018} & x &  &  &  &  &  &  &  &  &  & x & x &  &  & NR & 39 ppb & NR & 0.94 & 
         2.17 & 4.00 & 4.01 & 1.00 & 2.13 \\
         & FFNN & \cite{DeVito2009} & x &  &  &  &  &  &  & x &  &  &  &  &  &  & NR & 0.31 ppm & 27.00 \% & NR & 
         3.33 & 1.00 & 1.00 & 5.00 & 2.07 \\
         & RF & \cite{Borrego2018} & x & x & x &  & x & x & x &  &  & x & x & x &  &  & NR & 0.07 ppm & 280.00 \% & 0.88 & 
         1.00 & 1.00 & 3.60 & 2.57 & 1.43 \\
         & FFNN & \cite{Borrego2018} & x & x & x &  & x & x & x &  &  & x & x & x &  &  & NR & 0.09 ppm & 34.00 \% & 0.51 & 
         1.00 & 1.00 & 3.30 & 2.57 & 1.41 \\
         & LR & \cite{Saukh2015} & x &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.23 ppm & NR & NR & NR & 
         1.00 & 5.00 & 1.50 & 1.00 & 1.36 \\
        \hline
        \multirow{5}{*}{CO\textsubscript{2}} & FFNN & \cite{Spinelle2017} & x & x &  &  & x &  &  &  &  &  &  &  &  &  & NR & 2--18 & NR & 0.787 & 2.43 & 5.00 & 3.89 & 3.50 & 2.58 \\
         & RF & \cite{Zimmerman2018} & x & x &  &  & x & x &  &  &  &  & x & x &  &  & NR & 1.7 ppb & NR & 0.99 & 2.17 & 4.00 & 5.00 & 2.50 & 2.43 \\
         & MLR & \cite{Zimmerman2018} &  & x &  &  &  &  &  &  &  &  & x & x &  &  & NR & 19 ppb & NR & 0.49 & 2.17 & 4.00 & 3.65 & 3.00 & 2.24 \\
         & FFNN & \cite{Maag2018} &  &  &  &  &  & x &  & x &  &  & x &  &  &  & NR & 44 ppb & NR & 0.94 & 1.21 & 0.00 & 2.94 & 5.00 & 1.53  \\
         & MLR & \cite{Maag2018} &  &  &  &  &  & x &  & x &  &  & x &  &  &  & NR & 135 ppb & NR & 0.49 & 1.21 & 0.00 & 1.00 & 5.00 & 1.34 \\
        \hline
        \multirow{3}{*}{NO} & FFNN & \cite{Spinelle2017} &  &  & x &  & x &  &  &  &  &  & x & x &  &  & NR & 0.1--0.5 & NR & 0.208 & 2.43 & 5.00 & 5.00 & 3.00 & 2.75 \\
         & FFNN & \cite{Borrego2018} & x & x & x &  & x & x & x &  &  & x & x & x &  &  & NR & 2.39 ppb & 84.00 \% & 0.39 & 1.00 & 1.00 & 3.07 & 2.57 & 1.39 \\
         & RF & \cite{Borrego2018} & x & x & x &  & x & x & x &  &  & x & x & x &  &  & NR & 4.76 ppb & 127.00 \% & 0.74 & 1.00 & 1.00 & 1.00 & 2.57 & 1.22 \\
        \hline
        \multirow{15}{*}{NO\textsubscript{2}} & MLR & \cite{Maag2016} & x &  &  &  & x & x &  &  &  &  & x & x &  &  & 5.13 ppb & NR & NR & NR & 5.00 & 5.00 & 2.22 & 2.33 & 3.35 \\
         & RF & \cite{Zimmerman2018} & x & x &  &  & x & x &  &  &  &  & x & x &  &  & NR & 0.5 ppb & NR & 0.99 & 2.17 & 4.00 & 5.00 & 2.50 & 2.43 \\
         & FFNN & \cite{Spinelle2015} & x &  &  &  & x & x &  &  &  &  &  &  & x &  & NR & 2--4.5 ppb & NR & 0.596 & 2.43 & 5.00 & 3.30 & 3.00 & 2.42 \\
         & FFNN & \cite{DeVito2009} & x &  &  & x & x & x &  & x &  &  &  &  &  &  & NR & 10.1 ppb & 22.00 \% & NR & 3.33 & 1.00 & 1.00 & 5.00 & 2.07 \\
         & MLR & \cite{Zimmerman2018} &  &  &  &  & x &  &  &  &  &  & x & x &  &  & NR & 4.6 ppb & NR & 0.59 & 2.17 & 4.00 & 2.51 & 1.00 & 1.87 \\
         & TDNN & \cite{Esposito2016} &  &  & x &  & x & x &  &  &  &  & x & x &  &  & NR & 1.27 ppb & 22.00 \% & NR & 1.23 & 5.00 & 4.29 & 1.00 & 1.72 \\
         & NARX & \cite{Esposito2016} &  &  & x &  & x & x &  &  &  &  & x & x &  &  & NR & 1.30 ppb & 21.00 \% & NR & 1.23 & 5.00 & 4.28 & 1.00 & 1.72 \\
         & FFNN & \cite{Esposito2016} &  &  & x &  & x & x &  &  &  &  & x & x &  &  & NR & 1.50 ppb & 25.00 \% & NR & 1.23 & 5.00 & 4.20 & 1.00 & 1.71 \\
         & RF & \cite{Borrego2018} & x & x & x &  & x & x & x &  &  & x & x & x &  &  & NR & 1.97 ppb & 17.00 \% & 0.89 & 1.00 & 1.00 & 3.99 & 2.57 & 1.46 \\
         & FFNN & \cite{Borrego2018} & x & x & x &  & x & x & x &  &  & x & x & x &  &  & NR & 2.00 ppb & 25.00 \% & 0.81 & 1.00 & 1.00 & 3.98 & 2.57 & 1.46 \\
         & MLR & \cite{Cordero2018} &  &  & x &  & x & x &  &  &  &  & x &  &  &  & 2.92--3.88 ppb & 2.34--3.14 ppb & 12.3--35.4\% & 0.81--0.93 & 0.00 & 1.00 & 2.93 & 1.00 & 1.27 \\
         & RF & \cite{Cordero2018} &  &  & x &  & x & x &  &  &  &  & x &  &  &  & 2.29--4.73 ppb & 1.86--3.35 ppb & 16.0--32.9\% & 0.85--0.95 & 0.00 & 1.00 & 2.43 & 1.00 & 1.23 \\
         & SVM & \cite{Cordero2018} &  &  & x &  & x & x &  &  &  &  & x &  &  &  & 2.87--4.94 ppb & 2.07--4.36 ppb & 19.8--34.3\% & 0.79--0.95 & 0.00 & 1.00 & 2.32 & 1.00 & 1.23 \\
         & FFNN & \cite{Cordero2018} &  &  & x &  & x & x &  &  &  &  & x &  &  &  & 3.24--7.44 ppb & 2.76--6.22 ppb & 20.2--93.4\% & 0.62--0.88 & 0.00 & 1.00 & 1.34 & 1.00 & 1.15 \\
         & LR & \cite{Lin2015} &  &  &  &  & x &  &  &  &  &  &  &  &  &  & NR & NR & NR & 0.88 & 1.00 & 4.67 & 0.00 & 1.00 & 1.23 \\
        \hline
        \multirow{2}{*}{NO\textsubscript{x}} & TDNN & \cite{Esposito2016} &  &  & x &  & x & x &  &  &  &  & x & x &  &  & NR & 1.37 ppb & 20.00 \% & NR & 1.23 & 5.00 & 5.00 & 1.00 & 1.79 \\
         & FFNN & \cite{Esposito2016} &  &  & x &  & x & x &  &  &  &  & x & x &  &  & NR & 1.95 ppb & 29.00 \% & NR & 1.23 & 5.00 & 1.00 & 1.00 & 1.39 \\
        \hline
        \multirow{13}{*}{O\textsubscript{3}} & MLR & \cite{Maag2016} & x &  &  &  & x & x &  &  &  &  & x & x &  &  & 2.8 ppb & NR & NR & NR & 5.00 & 5.00 & 3.82 & 2.33 & 4.00 \\
         & FFNN & \cite{Spinelle2015} & x &  &  &  & x & x &  &  &  &  &  &  &  &  & NR & 1--4.5 ppb & NR & 0.915 & 2.43 & 5.00 & 3.84 & 2.33 & 2.46 \\
         & RF & \cite{Zimmerman2018} & x & x &  &  & x & x &  &  &  &  & x & x &  &  & NR & 0.7 ppb & NR & 0.99 & 2.17 & 4.00 & 5.00 & 2.50 & 2.43 \\
         & MLR & \cite{Zimmerman2018} &  &  &  &  &  & x &  &  &  &  & x & x &  &  & NR & 5.1 ppb & NR & 0.81 & 2.17 & 4.00 & 2.93 & 5.00 & 2.29 \\
         & LR & \cite{Hasenfratz2012} &  &  &  &  &  & x &  &  &  &  &  &  &  &  & NR & 1.46 ppb & NR & NR & 1.00 & 5.00 & 4.24 & 5.00 & 1.74 \\
         & FFNN & \cite{Maag2018} &  &  &  &  &  & x &  & x &  &  & x &  &  &  & NR & 3.5 ppb & NR & 0.91 & 1.21 & 0.00 & 3.57 & 5.00 & 1.59 \\
         & TDNN & \cite{Esposito2016} &  &  & x &  & x & x &  &  &  &  & x & x &  &  & NR & 7.45 ppb & 42.00 \% & NR & 1.23 & 5.00 & 2.05 & 1.00 & 1.50 \\
         & RF & \cite{Borrego2018} & x & x & x &  & x & x & x &  &  & x & x & x &  &  & NR & 1.32 & 20.00 \% & 0.97 & 1.00 & 1.00 & 4.28 & 2.57 & 1.49 \\
         & FFNN & \cite{Esposito2016} &  &  & x &  & x & x &  &  &  &  & x & x &  &  & NR & 7.90 ppb & 70.00 \% & NR & 1.23 & 5.00 & 1.91 & 1.00 & 1.48 \\
         & LR & \cite{Saukh2015} &  &  &  &  &  & x &  &  &  &  &  &  &  &  & 12.9 ppb & NR & NR & NR & 1.00 & 5.00 & 1.00 & 5.00 & 1.48 \\
         & FFNN & \cite{Borrego2018} & x & x & x &  & x & x & x &  &  & x & x & x &  &  & NR & 2.60 ppb & 18.00 \% & 0.86 & 1.00 & 1.00 & 3.89 & 2.57 & 1.45 \\
         & LR & \cite{Lin2015} &  &  &  &  &  & x &  &  &  &  &  &  &  &  & NR & NR & NR & 0.92 & 1.00 & 4.67 & 0.00 & 5.00 & 1.39 \\
         & MLR & \cite{Maag2018} &  &  &  &  &  & x &  & x &  &  & x &  &  &  & NR & 10.7 ppb & NR & 0.16 & 1.21 & 0.00 & 1.29 & 5.00 & 1.37 \\
        \hline
        \multirow{3}{*}{PM\textsubscript{2.5}} & FFNN + GP & \cite{Cheng2014} &  &  &  &  &  &  &  &  & x &  & x & x &  &  & 96.69 ug/m\textsuperscript{3} & NR & NR & NR & 1.67 & 5.00 & 5.00 & 4.00 & 2.27 \\
         & MLR & \cite{Liu2017a} &  &  &  &  &  &  &  &  & x &  &  &  &  & x & NR & NR & NR & 0.9959 & 1.02 & 5.00 & 0.00 & 4.00 & 1.37 \\
         & FFNN + GP & \cite{Gao2016} &  &  &  &  &  &  &  &  & x &  & x & x &  &  & NR & NR & 5.40 \% & NR & 0.00 & 5.00 & 0.00 & 4.00 & 1.00 \\
        \hline
        \multirow{2}{*}{SO\textsubscript{2}} & RF & \cite{Borrego2018} & x & x & x &  & x & x & x &  &  & x & x & x &  &  & NR & 0.09 ppb & 5.00 \% & 0.95 & 1.00 & 1.00 & 5.00 & 2.57 & 1.54 \\
         & FFNN & \cite{Borrego2018} & x & x & x &  & x & x & x &  &  & x & x & x &  &  & NR & 0.16 ppb & 10.00 \% & 0.86 & 1.00 & 1.00 & 1.00 & 2.57 & 1.22 \\
        \bottomrule
    \end{tabular}}
\end{sidewaystable*}

==> tables/ml-spatio-temporal.tex <==
\begin{table*}[!ht]
    \centering
    \caption{Spatio-temporal models for AQSs}
    \label{tab:ml-spatio-temporal}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccc|ccc}
       \hline
        ML & \multicolumn{3}{c|}{Gas sensors} & \multicolumn{3}{c}{PM} \\
        & CO & NO\textsubscript{2} & O\textsubscript{3} & PM\textsubscript{2.5} & PM\textsubscript{10} & UFP \\
        \hline
        \hline
        LR & \cite{Hu2016} & & & & & \\
        \hline
        \multirow{2}{*}{SVR} & \cite{Hu2016} & & & & & \\
         & \cite{Hu2017} & & & & & \\
        \hline
        DT & \cite{Hu2017} & & & & & \\
        \hline
        RF & \cite{Hu2017} & & & & & \\
        \hline
        AdaBoost & \cite{Hu2017} & & & & & \\
        \hline
        XGBoost & \cite{Hu2017} & & & & & \\
        \hline
        LUR & & & & & & \\
        \hline
        GAMS & \cite{Hasenfratz2014} & & \cite{Hasenfratz2014} & & & \cite{Hasenfratz2014} \\
        \hline
        GP & & \cite{Chen2016} & &  \cite{Chen2016} & \cite{Chen2016} &  \\ 
    \end{tabular}
    }
\end{table*}

